End-to-end Modeling and Optimization of Timing and Energy in Wireless IoT Systems

With the advent of edge computing, data generated by end devices can be pre-processed before transmission, possibly saving transmission time and energy. On the other hand, data processing itself incurs latency and energy consumption, depending on the complexity of the computing operations and the speed of the processor. The energy-latency-reliability profile resulting from the concatenation of pre-processing operations (specifically, data compression) and data transmission is particularly relevant in wireless communication services, whose requirements may change dramatically with the application domain. In this paper, we study this multi-dimensional optimization problem, introducing a simple model to investigate the tradeoff among end-to-end latency, reliability, and energy consumption when considering compression and communication operations in a constrained wireless device. We then study the Pareto fronts of the energy-latency trade-off, considering data compression ratio and device processing speed as key design variables. Our results show that the energy costs grows exponentially with the reduction of the end-to-end latency, so that considerable energy saving can be obtained by slightly relaxing the latency requirements of applications. These findings challenge conventional rigid communication latency targets, advocating instead for application-specific end-to-end latency budgets that account for computational and transmission overhead.

==> acronyms.tex <==
\newacronym{ts}{TS}{Time Sensitive}
\newacronym{aoi}{AoI}{Age of Information}
\newacronym{voi}{VoI}{Value of Information}
\newacronym{qaoi}{QAoI}{Query Age of Information}
\newacronym{bs}{BS}{Base Station}
\newacronym{harq}{HARQ}{Hybrid Automated Repeat Request}
\newacronym{ee}{EE}{Energy Efficiency}
\newacronym{adc}{ADC}{Analog to Digital Converter}
\newacronym{urllc}{URLLC}{Ultra Reliable Low Latency Communication}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{pdf}{PDF}{Probability Density Function}
\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{kpis}{KPIs}{Key Performance Indicators}
\newacronym{snr}{SNR}{Signal to Noise Ratio}
\newacronym{arq}{ARQ}{Automatic Repeat Request}
\newacronym{iid}{iid}{independent and identically distributed}
\newacronym{5g}{$\textrm{5}$G}{fifth-generation}
\newacronym{6g}{$\textrm{6}$G}{sixth-generation}
\newacronym{cpu}{CPU}{central processing unit}
\newacronym{spa}{SPA}{Saddle Point Approximation}


==> schemes/first_scenario_new.tex <==
\begin{tikzpicture}[>=stealth,thick]
  % axes
  \draw[->] (-3,0) -- (3,0) node[pos=1.0, below] {$t$ [s]};
  \draw[->] (-3,0) -- (-3, 1.5) node[pos=0.9, left] {$B$ [Hz]};

  % blocks
  \draw[draw=black, fill=cComp] (-2,0) rectangle (-0.7,0.7)
    node[pos=.5, text=black] {$T_c$};
  \draw[draw=black, fill=cTx] (-0.7,0) rectangle (1,0.7)
    node[pos=.5, text=black] {$T_{\mathrm{tx}}$};
  \draw[draw=black, fill=cDecomp] (1,0) rectangle (1.6,0.7)
    node[pos=.5, text=black] {$T_d$};

  % callouts
  \draw[->] (-2.5,-0.4) -- (-2,0) node[pos=.0, below] {Compression starts};
  \draw[->] (-0.9,-0.8) -- (-0.7,0) node[pos=.0, below] {Transmission starts};
  \draw[->] (0.6,-0.4) -- (1,0) node[pos=.0, below] {Data received};
  \draw[->] (2.0,-1.2) -- (1.6,0) node[pos=.0, below] {Decompressed};

  \draw[->] (-2,1.5) -- (-2,0.35) node[pos=.0, above] {Data requested};
  \draw[->] (1.6,0.35) -- (1.6,1.5) node[pos=1.0, above] {Data delivered};

  % brace for E2E latency
  \draw [decorate,decoration={brace,amplitude=5pt,raise=-3ex}]
    (-2,1.3) -- (1.6,1.3) node[midway, yshift=1pt]{End-to-end Latency};
\end{tikzpicture}


==> schemes/second_scenario_new.tex <==
% ----- In your frame -----
\begin{tikzpicture}[>=stealth,thick]

  % Axes (one for computation row, one for communication row)
  \draw[->] (-3,0.5) -- (3,0.5) node[pos=1.0, below] {$t$ [s]};
  \node[anchor=east] at (-3,1.3) {\small Computation};

  \draw[->] (-3,2) -- (3,2) node[pos=1.0, below] {$t$ [s]};
  \node[anchor=east] at (-3,2.8) {\small $B$ [Hz]};

  % Time slots on the communication row (top row)
  \draw[draw=black, fill=cSlot] (-2.5,2) rectangle (-0.7,2.7)
    node[pos=.5] {\small TS 1};
  \draw[draw=black, fill=cTx] (-0.7,2) rectangle (1.0,2.7)
    node[pos=.5] {\small TS 2};
  \draw[draw=black, fill=cSlot] (1.0,2) rectangle (2.7,2.7)
    node[pos=.5] {\small TS 3};

  % Computation row: compression and decompression bars
  \draw[draw=black, fill=cComp] (-2.0,0.5) rectangle (-0.9,1.0)
    node[pos=.5] {$T_c$};
  \draw[draw=black, fill=cComp] (1.0,0.5) rectangle (1.6,1.0)
    node[pos=.5] {$T_d$};

  % Vertical guides (slot boundaries)
  \draw[dashed] (-2.0, 3) -- (-2.0, 0);
  \draw[dashed] (-0.7, 3) -- (-0.7, 0);
  \draw[dashed] ( 1.0, 3) -- ( 1.0, 0);
  \draw[dashed] ( 1.6, 3) -- ( 1.6, 0);

  % Callouts
  \draw[->] (-2.5,0.1) -- (-2.0,0.5) node[pos=0, below] {\small Compression starts};
  \draw[->] (-0.9,-0.3) -- (-0.7,0.5) node[pos=0, below] {\small Transmission starts};
  \draw[->] (0.6,0.1) -- (1.0,0.5) node[pos=0, below] {\small Data received};
  \draw[->] (2.0,-0.6) -- (1.6,0.5) node[pos=0, below] {\small Data decompressed};

  % Braces and labels
  % Compression window (alpha T)
  \draw[decorate,decoration={brace,amplitude=5pt}]
    (-2.0,1.5) -- (-0.7,1.5)
    node[midway, below=3pt] {$T_{\mathrm{comp}}=\alpha T$};

  % Transmission slot ((1-alpha)T)
  \draw[decorate,decoration={brace,amplitude=5pt}]
    (-0.7,1.5) -- (1.0,1.5)
    node[midway, below=3pt] {$T_{\mathrm{slot}}=(1-\alpha)T$};

  % Total horizon T (from compression start to end of TX slot)
  \draw[decorate,decoration={brace,amplitude=5pt}]
    (-2.0,3.2) -- (1.0,3.2)
    node[midway, above=6pt] {$T$};

\end{tikzpicture}

